Real-Time Reduced-Order Modeling of Stochastic Partial Differential Equations via Time-Dependent Subspaces

We present a new methodology for the real-time reduced-order modeling of stochastic partial differential equations called the dynamically/bi-orthonormal (DBO) decomposition. In this method, the stochastic fields are approximated by a low-rank decomposition to spatial and stochastic subspaces. Each of these subspaces is represented by a set of orthonormal time-dependent modes. We derive exact evolution equations of these time-dependent modes and the evolution of the factorization of the reduced covariance matrix. We show that DBO is equivalent to the dynamically orthogonal (DO) and bi-orthogonal (BO) decompositions via linear and invertible transformation matrices that connect DBO to DO and BO. However, DBO shows several improvements compared to DO and BO: (i) DBO performs better than DO and BO for cases with ill-conditioned covariance matrix; (ii) In contrast to BO, the issue of eigenvalue crossing is not present in the DBO formulation; (iii) In contrast to DO, the stochastic modes are orthonormal, which leads to more accurate representation of the stochastic subspace. We study the convergence properties of the method and compare it to the DO and BO methods. For demonstration, we consider three cases: (i) stochastic linear advection equation, (ii) stochastic Burgers' equation, and (iii) stochastic incompressible flow over a bump in a channel. Overall we observe improvements in the numerical accuracy of DBO compared against DO and BO.

==> Sections/Lemma3.tex <==
\begin{enumerate}[label=(\roman*)]
 \item \begin{equation*}
      {U}_{DO} =  {U}_{BO}  {W}_{u_{eq}}.
 \end{equation*}
 Using the equivalence between DO with DBO and BO with DBO i.e., Lemma (\ref{lemma1}) and (\ref{lemma2}) in the above equation, we get: 
 \begin{equation*}
      {U}_{DBO}  {R}_u =  {U}_{DBO}  {W}_u  {W}_{u_{eq}}.
 \end{equation*}
Projecting the above equation on the DBO spatial basis and using the orthonormality property of the basis i.e., $\left<U_{DBO}, U_{DBO} \right> = I$, the equation simplifies to
 \begin{align*}
  \left< U_{DBO}, U_{DBO} \right> {R}_u &= \left< U_{DBO}, U_{DBO} \right>  {W}_u  {W}_{u_{eq}}, \\
      {W}_{u_{eq}} &=  {W}_u^{-1}  {R}_u.
 \end{align*}
 \item Similarly for the stochastic modes,
 \begin{equation*}
      {Y}_{DO} =  {Y}_{BO}  {W}_{y_{eq}}.
 \end{equation*}
 Once again using the equivalence between DO with DBO and BO with DBO i.e., Lemma (\ref{lemma1}) and (\ref{lemma2}) in the above equation, we get: 
 \begin{equation*}
      {Y}_{DBO}  {W}_y =  {Y}_{DBO}  {R}_y  {W}_{y_{eq}}.
 \end{equation*}
 Taking expectation after pre-multiplying with $ {Y}_{DBO}^T$ and using the orthonormality property of the stochastic modes, we get:
 \begin{equation*}
      {W}_{y_{eq}} =  {R}_y^{-1}  {W}_y.
 \end{equation*}
\end{enumerate}
This completes the proof. 
